Fighting Selection Bias in Statistical Learning: Application to Visual Recognition from Biased Image Databases

In practice, and especially when training deep neural networks, visual recognition rules are often learned based on various sources of information. On the other hand, the recent deployment of facial recognition systems with uneven performances on different population segments has highlighted the representativeness issues induced by a naive aggregation of the datasets. In this paper, we show how biasing models can remedy these problems. Based on the (approximate) knowledge of the biasing mechanisms at work, our approach consists in reweighting the observations, so as to form a nearly debiased estimator of the target distribution. One key condition is that the supports of the biased distributions must partly overlap, and cover the support of the target distribution. In order to meet this requirement in practice, we propose to use a low dimensional image representation, shared across the image databases. Finally, we provide numerical experiments highlighting the relevance of our approach.

==> acknowledgments.tex <==
This research work was partially supported
by the research chair ``Good In Tech :
Rethinking innovation and technology as
drivers of a better world for and by humans``,
under the auspices of the ''Fondation du Risque``
and in partnership with the
Institut Mines-Télécom, Sciences Po, Afnor, Ag2r La
Mondiale, CGI France, Danone and Sycomore.


==> expe_old.tex <==
\iffalse
% Old proposition of dataset generation


\robin{TODO: Correct this.}
We chose to split the dataset into $K$ pieces that cover distinct parts of the space.
Also, we impose that only one class is significantly represented in every pair of datasets,
\textit{i.e.} $p_k(y) = \sqrt{\gamma}$ and $p_l(y) = \sqrt{\gamma}$
for some $y \in \mathcal{Y}$
and $p_k(y')p_l(y') = 0$ for any $y' \ne y$,
where $\gamma$ is a fixed parameter.
In practice, for some permutation of the classes $\sigma \in \mathfrak{S}_Q$
with $Q = \# \mathcal{Y}$,
we can write $Q = a K + (K-1) + r$ with $(a, r) \in \mathbb{N}
\times \llbracket 1, K - 1\rrbracket$
as soon as $Q \ge K-1$. Then we assign all observations
that satisfy $y_i \le a$ to $\mathcal{D}_1$
and elements that satisfy $y_i = a+1$ with proportion $\sqrt{\gamma}$.
We assign the same proportion to $\mathcal{D}_2$ of elements satisfying
$y_i = a+1$ and assign all observations such that $y_i \in [a+2, 2a+1]$.
Following this idea, we continue ``linking'' sequentially the datasets
with an intermediary class.
The last dataset $\mathcal{D}_K$ contains all of the $r$ remaining classes.
If the dataset $\mathcal{D}_k$ contains $C$ ``complete'' classes and is at the side,
we have $p_k(y) = (1-\sqrt{\gamma})/C$ for any central class,
$p_k(y) = \sqrt{\gamma}$ for a side class and $p_k(y) = 0$ for any other class.
Any bias function $\omega$ proportional to these values is appropriate.
We illustrate the number of elements per class for all datasets
in a scenario where $K=5$ in \cref{fig:synthetic_example}.
\robin{TODO: make this clearer.}
We limit the number of training observations to 30K so that all experiments feature
the same number of training observations, regardless of the value of $\gamma$.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/generated_distribution.pdf}
    \caption{Number of element per class for all datasets in a scenario where
	$K = 5$ and $\gamma$ is either high (0.2) or low (0.01)
	and the classes are not permuted, for both CIFAR10 ($Q = 10$)
	and CIFAR100 ($Q=100$).
	\robin{TODO: Remove the left ``low gamma'' / ``high gamma''
	and precise that in the caption. Make fonts more readable.}
    }\label{fig:synthetic_example}
\end{figure}

% Old proposition learning with noisy bias functions

In practical scenarios, the true biasing functions $\omega_k$'s are deduced from
empirical estimates of the proportions, thus are not exact proportions.
More generally, the biasing functions could often be an informed guess,
rather than accurate information on the distributions.
For this reason, we study the expected loss of accuracy when injecting noise
into the value of the bias function. In practice, we replace the true values
$\omega_k(y)$ by $\rho_k(y) = \omega_k(y) + \lambda \cdot \xi_k$
where $\xi_k$ is a term from from $n$-dimensional Dirichlet distribution
with parameters $(1, \dots, 1)$ and $\lambda \in \R$.
Results are provided in \cref{fig:accuracy_vs_noise}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\columnwidth]{figures/exps/noise_plot_cifar10.pdf}
    \includegraphics[width=0.49\columnwidth]{figures/exps/noise_plot_cifar100.pdf}
    \caption{
	Accuracy as a function of the noise proportion. The x markers denote the bottom and
	top of a 95\% confidence interval for the learning problem.
	\robin{TODO: Same remark as \cref{tab:table_accs}}
    }\label{fig:accuracy_vs_noise}
\end{figure}

% Old second experiment

In this scenario, we assume that we have
access to a small dataset $\mathcal{D}_{\text{test}} = \left\{ (x_1', y_1'),
\dots, (x'_{n_{\text{test}}}, y'_{n_{\text{test}}}) \right\}$. 
We propose to learn a first model $f\circ g$ on the concatenation of all
datasets $\mathcal{D}_1, \dots, \mathcal{D}_K$, then to fit a mixture 
of Gaussian model on the encoding of $\mathcal{D}_{\text{test}}$
and use the estimated proportions over each $\mathcal{D}_k$ to approximate
the biasing functions. Finally, we learn the final model from scratch
using the obtained sampling weights.

\textbf{Synthetic biased datasets.}
To provide a small testing sample, we set aside some of the training data,
without changing its distribution.
We propose to generate the synthetic training datasets using the strategy proposed in
\cref{subsec:exp:bias_fun} as well as random assignment.
Finally we propose to use a random linear classifier on a simple transformation
of the images, namely the concatenation of the average color value of the top-left,
top-right, bottom-left and bottom-right of the image.


\textbf{From Gaussian model to bias functions.}
We fit a Gaussian model with $L$ components on a small
$\mathcal{D}_{\text{test}}$ and predict the
average probability over the different components $q_{\text{test}} \in \R^L$
of that Gaussian model.
Finally, the bias term is 
\begin{align*}
    \omega_k(x) = q \cdot \frac{q_\text{test}}{q^{k} + \epsilon},
\end{align*}
where $q$ is the predicted probabilities in $\R^L$, $q^{(k)} \in \R^L$
are the average probabilities of dataset $k$ for the Gaussian mixture model
and $q_{\text{test}} \in \R^L$ is the average probabilities of the test set
for the mixture model.
\robin{Is there a better way? to discuss.}

\textbf{Size of the encoding and biasing complexity.}
In \cref{fig:exp_heatmap_size_encoding}, we plot the obtained testing accuracy
as a function of the number of different Gaussian components in the mixture model,
for three different imbalance scenarios.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/placeholder.jpg}
    \caption{\robin{TODO}}\label{fig:exp_heatmap_size_encoding}
\end{figure}

\begin{table}[t]
    \centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{ccccc}
	\toprule
	CIFAR10 & \multicolumn{4}{l}{Base accuracy $92.93 \; (\pm 0.47)$} \\
	\midrule
	$\gamma$ & 0.001 & 0.01 & 0.10 & 0.20 \\
	Acc. & $89.96 \;(\pm 2.15)$ &
	$90.51 \;(\pm 1.72)$ & $90.97 \; (\pm 1.64)$ & $91.02 \; (\pm 1.64)$ \\
	\midrule
	\midrule
	CIFAR100 & \multicolumn{4}{l}{Base accuracy $69.77 \;(\pm 1.12)$} \\
	\midrule
	$\gamma$ & 0.001 & 0.01 & 0.10 & 0.20 \\
	Acc. & $62.00 \; (\pm 6.73)$ & $63.66 \; (\pm 3.66)$ & $65.08 \; (\pm 0.74)$
	& $64.96 \; (\pm 1.96)$ \\
	\bottomrule
    \end{tabular}}
    \smallskip
    \caption{Accuracies for different $\gamma$'s on CIFAR10 and CIFAR100,
	with 2 times the standard deviation over 8 runs between parenthesis.
    }\label{tab:table_accs}
\end{table}

\fi


==> extra_content.tex <==
\robin{Relate that setting with the Example 1 of P. Laforgue and Clemençon
on Statistical Biased Samples.}

\robin{When confronted with a dataset, is it a reweighting of the data or a censored
    version of a full dataset ?}

\section{Related work}

\cite{HendricksBSDR18}: Proposes an Equalizer model for caption,
that uses masks on persons to learn to derive the gender information
from the information contained in the person.
Builds a database from the captions given with MsCOCO.

\cite{ZhangYCW15}: Proposes to consider transfer learning as modelling
the difference between conditional distributions and marginal distributions
independently, does so with the MMD loss, which boils down to simple distances
between averages. Uses an iterative procedure to generate target labels.
It is a bad arxiv paper, that wasn't published at a major conference.

\cite{GaninJMLR}: Propose to perform domain adaptation by backpropagation,
uses a gradient reversal layer to confuse a domain classifier.
Contains many interesting references for domain adaptation and transfer learning.
One idea would be to integrate the estimation of the $W_k$'s in the learning process,
while at the same time trying to learn shared features,
to make our probabilistic modelling more relevant.

\cite{Tzeng2015}: Proposes to perform transfer learning using a loss to maximize
domain confusion, as well as a loss that transfers the correlation between tasks,
using a small set of labeled instances in the target set, that may not contain
some classes that are present in the source data.

\cite{NIPS2009_3666}: Proposes using a loss that includes distribution
matching with MMD to perform transduction (reasoning from observed, specific
    train cases, to specific test cases, while induction reasons
from train cases to rules, that are applied later on test data).
In this work, we consider learning with several biased datasets
sually we perform induction in ML, by learning some model.

\cite{LiYSH18}: Proposes to tackle the problem of Domain Generalization (DG),
not Domain Adaptation (DA). For that, it learns an algorithm (MLDG) that tries and 
obtains good performance on two different sets of the training data
and assures that the gradient are aligned, with a specific loss.
Precisely, where $\mathcal{F}$ is the loss on part of the source datasets
and $\mathcal{G}$ on another part:
\begin{align*}
    \arg\min_{\Theta} \mathcal{F}(\Theta)
    + \beta  \mathcal{G}(\Theta - \alpha \mathcal{F}'(\Theta)).
\end{align*}
The explanation as to why it requires aligned gradients between $\mathcal{F}$ and 
$\mathcal{G}$ can be found in the paper.

\cite{LongZ0J16}: Proposes Residual Transfer Networks, which include a loss that
write:
\begin{align*}
    \min_{f_s = f_T + \Delta f} \frac{1}{n_s} \sum_{i=1}^{n_s} L(f_s(x_i^s), y_i^s)
    + \frac{\gamma}{n_t} \sum_{i=1}^{n_t} H(f_t(x_i^t))
    + \lambda D_{\mathcal{L}}(\mathcal{D}_s, \mathcal{D}_t),
\end{align*}
where $L(f_s(x_i^s), y_i^s)$ is the usual source loss, $H(f_t(x_i^t))$ is an entropy loss,
which favors results with binary output on the target domain, and $\mathcal{D}_{\mathcal{L}}$
is composed of the MMD between the distribution of the encoded features.
The paper features an extensive presentation of different domain adaptation
contributions, as well as the consideration that transfering deep features
is not all that matters.

\cite{BousmalisTSKE16}: Consider a lot of different elements and different losses.
It learns a component that is invariant between domains, as well as a component that
is specific to each domain.
\cite{BousmalisTSKE16} considers reconstruction losses so I will just not consider it
here.

\robin{Talk about the related work:

    Surveys on Transfer Learning:
    \begin{itemize}
	\item \cite{ASurveyTransferLearning} on transfer learning, a bit old,
	\item \cite{SurveyOnTransferLearningBigData} on transfer learning,
	    maybe too high level for us,
	\item \cite{tan2018survey} insufferably poorly written, but may
	    contain good references,
    \end{itemize}

}

\section{Former writing}

\textbf{Probabilistic framework.}
% Introduction du point de vue probabiliste sur la classification
From a probabilistic point of view, a natural way to consider
visual recognition tasks is in the setting of multiclass classification.
The (multi-class) classification setting introduces a random
variable $Y$ that denotes the output label with values in the
discrete set $\Y := \{ 1, \dots, L\}$ with $L \ge 1$,
as well as the input random variable $X$,
with values in a feature space $\X \subset \R^d$ with $d \ge 1$.
We Denote by $Z := (X, Y)$ the pair composed of the random variables
$X$ and $Y$ with values in the product space $\Z := \X \times \Y$,
and introduce its distribution by $P$.

\textbf{Empirical risk minimization (ERM).}
Introduce a classifier $g_\theta: \X \to \Y$ parameterized
by some $\theta \in \Theta$.
The usual goal of classification is to minimize an expected
classification risk $L_{Z \sim P}(\theta) := \p\{ g_\theta(X) \ne Y\}$
with target distribution $P$ over the parameter space $\Theta$,
\textit{i.e.} to solve
\begin{align}\label{eq:Expected_risk}
    \min_{\theta\in\Theta} L_P(\theta).
\end{align}
For the class of all measurable functions, an analytical expression
of an optimal classifier exists for \cref{eq:Expected_risk} (see \cite{Devroye1996}),
but it depends on the unknown posterior probabilities
$\eta_k : x \mapsto \p\{ Y = k \mid X = x \}$ for all $k \in \{1, \dots, K \}$.
Therefore, finding a good solution to \cref{eq:Expected_risk} usually relies
on the principle of Empirical Risk Minimization (ERM).
In its simplest form, ERM assumes the existence of an independent
and identically distributed (\textit{i.i.d.}) training sample
$\mathcal{D}_n = \{ (X_1, Y_1), \dots, (X_n, Y_n) \}$ of $n$ elements,
that follows the target distribution $P$. % Formally, we have $(X_1, Y_1) \sim P$.
The training sample then serves to derive an unbiased empirical estimator
$\widehat{L}_n(g_\theta) = (1/n) \sum_{i=1}^n \I\{ g_\theta(X_i) \ne Y_i\}$
of the true risk $L_P(g_\theta)$.
If the estimator $\widehat{L}_n(g_\theta)$ enjoys good statistical properties,
minimizing $\widehat{L}_n(g_\theta)$ over $\Theta$ provides
reasonable solutions to \cref{eq:Expected_risk}.
The generalization properties of empirical minimizers of $\widehat{L}_n(g_\theta)$
was extensively covered by the statistical machine learning literature \cite{Boucheron2005}.


\textbf{Learning with several biased samples.}
The work of \cite{laforgue2019statistical}
relaxes the usual assumption that the distribution
of the training data corresponds to that of the target distribution $P$.
Precisely, they assume the existence of $K$ independent \textit{i.i.d}
training samples, defined as
$\mathcal{D}^{(k)}_{n_k} = \{ Z_1^{(k)}, \dots, Z_{n_k}^{(k)} \} \subset \mathcal{Z}$
with observations $Z_i^{(k)}$'s that follow the distribution $P^{(k)}$
for any $k \in \{ 1, \dots, K \}$.
Additionally, they assume that for any $k \in \{1, \dots, K\}$
the distribution $P^{(k)}$ satisfies $P^{(k)} \ll P$,
where $\mu \ll \lambda$ denotes the absolute continuity of a measure
$\mu$ with respect to another measure $\lambda$ \cite[Definition 1.3]{Shorack2000}.
Under that assumption, there exists a Radon-Nikodym derivative for $P_k$ with respect to $P$,
which means that there is an analytical expression for 
writing $P_k$ as a reweighted version of the distribution $P$.
We refer to \cite[Theorem 2.3]{Shorack2000} for more technical details.
Following the notations of \cite{gill1988}, we introduce the \textit{biasing function}
$\omega^{(k)}$, that satisfies
\begin{align}\label{eq:baising-function}
    \forall z \in \Z, \; \frac{dP^{(k)}}{dP}(z) = \frac{\omega^{(k)}(z)}{\Omega^{(k)}},
\end{align}
where $\Omega^{(k)} = \E_{Z \sim P}[\omega^{(k)}(Z)]
= \int_{\mathcal{Z}} \omega^{(k)}(z) P(dz)$.
Under technical assumptions on the supports $\mathcal{Z}^{(k)} := 
\{ z \in \Z \mid \omega^{(k)}(z) > 0 \}$
of the biasing functions $\omega^{(k)}$'s for any $k \in \{ 1, \dots, K\}$,
\cite{gill1988} proposed reweighting the instances
in the datasets $\mathcal{D}^{(k)}$ to form an empirical distribution
$\widehat{P}_n$ that is unbiased with respect to $P$.
Their technique is based on empirical estimators for the $\Omega_k$'s that are
obtained by solving the system of equations (5) in \cite{laforgue2019statistical}.
However, it assumes that the values of the biasing functions $\omega_k$'s
on the elements of the training datasets are known, which is rarely the
case, unless those have a very special expression, see
\cite[Example 1]{laforgue2019statistical}.

\textbf{Auxiliary image data as biasing functions.}
\robin{Why is it known approximately ?}

% \input{subfiles/appendix.tex}
% \input{subfiles/rejected.tex}

\section{Former writing - Old experiments}

Following in the footsteps of \cite{vogel2020weighted},
we present an experiment that leverages the structure of the well-known
ImageNet Large Scale Visual Recognition Challenge (ILSVRC)
dataset to illustrate learning with several samples
with different distributions.
%introduced in \Cref{sec:stratified_population}.
% The code of the experiments can be found at
% \url{https://tinyurl.com/qwthb9q} (Google drive).
The ILSVRC challenge consists in
learning a classifier from 1.3 million training images spread out over 1,000
classes. Performance is evaluated using the validation dataset of 50,000
images of ILSVRC as our test dataset. ImageNet is an image database
organized according to the WordNet hierarchy, which groups nouns in sets
of related words called synsets. In that context, images are examples of
very precise nouns, e.g. \emph{flamingo}, which are contained in a larger
synset, e.g. \emph{bird}.
% Introduce the preprocessing of the data - encoding over ResNet50
The impact of reweighting in presence of strata bias
is illustrated on the ILSVRC classification problem with broad significance synsets for strata.
To do this, we encode the data using deep neural networks.
Specifically our encoding is the flattened output of the last convolutional
layer of the network ResNet50 introduced in \cite{DBLP:journals/corr/HeZRS15}.
It was trained for classification on the training dataset of ILSVRC.
% Introduce the strata, and the strata weights
A total of 33 strata are derived from a list of high-level categories provided
by ImageNet at \url{http://www.image-net.org/about-stats}.
\robin{Missing sentence\dots}
Leveraging the abundance of train data, we discarded elements
of the train set in each strata in a way that induces a parameterized strata biais.

We report significantly
better performance when reweighting using the strata information, compared to
the case where the strata information is ignored (Unif.).
For comparison, we added two reference experiments: one which reweights the
train instances by the class probabilities (Class), which we do not know in a
stratified population experiment, and one with more data and no strata bias
(No bias) because it uses all of the ILSVRC train data.
Tests with a multilayer perceptron (MLP) did not perform as well, see the code
\robin{Detail if necessary}.

\section{How are tasks labeled in papers}

\textbf{Domain Adaptation/Generalization.}
\cite{GaninJMLR} tries to find invariant representations of the data.
\cite{ParametrizationMultiDomainCVPR}
\cite{ZhangYCW15}
\cite{LongZ0J16}
\cite{BousmalisTSKE16}

Domain Generalization \robin{How it utilizes multiple sources}
\cite{LiYSH18}

\textbf{Transfer Learning.}
\cite{Tzeng2015}
\cite{GuoSKGRF19}
\cite{CuiSSHB18}
\cite{GeY17}
\cite{Ngiam2018}
\cite{49330}


\cite{Tzeng2015} does not only try to find invariant representations of the data.
\cite{BousmalisTSKE16} neither.


\robin{Introduce transfer learning as a way to learn with dataset bias,
present the general idea of transfer learning: and how most papers decompose them}

\robin{I can use \cite{ZamirSSGMS18} to draw inspiration for my related work section.}

\robin{\cite{GuoSKGRF19} to draw inspiration for my related work section.}
If I remember correctly, this paper cited different papers depending on the 
type of adaptation (last layers, all layers, etc\dots)

A lot of interesting references are contained in \cite{Zhu2020}, published in ECCV 2020.

On carefully selecting which input samples are relevant for the input task,
as in \cite{GeY17}

EMD quantifies domain similarity
\cite{CuiSSHB18}

Domain adaptive transfer learning (DATL) employs probabilistic shaping,
where the value is proportional to the ratios of estimated label prior probabilities.
\cite{Ngiam2018} (only arxiv paper)
(maybe add that and the arxiv paper that considers the priors and conditional distributions)

In \cite{Zhu2020}, some bias is derived from a scaling function.
They consider sample-independent modelling of the importance 
function $\lambda$ as in \cite{Ngiam2018}.

a common assumption is that the bias originates from low-level features,
as those capture variations due to factors such as resolution, illumination
and color \cite{BousmalisTSKE16}.

Explain why \citet{Kim_2019_CVPR} is less general than our setting.

\robin{To read \cite{Ben-DavidBCKPV10}}

\section{Old appendix}

\subsection*{Importance of reweighting for simple distributions}

% Introduce a random pair $(X,Y) \in \X \times \{-1, +1\}$ where $X \mid Y=+1$ follows
% a $\mathcal{N}(\mu_+, \sigma_+^2)$ and $X\mid Y=-1$ follows a $\mathcal{N}(0, 1)$,
% where $\mathcal{N}(\mu,\sigma^2)$ is a normal law of means $\mu$ and variance $\sigma^2$.
Introduce a random pair $(X,Y)$ in $[0,1] \times \{-1, +1\}$ where $X\mid Y=+1$
has for probability density function (pdf) $f_+(x) = ( 1 + \alpha ) x^\alpha, \alpha>0$ and
$X\mid Y=-1$ has for pdf $f_-(x) = ( 1 + \beta
)(1-x)^\beta, \beta>0$. As in \Cref{sec:background}, the train and test datasets have
different class probabilities $p'$ and $p$ for $Y=+1$.
The loss $\ell$ is defined as $\ell(\theta,z) = \I\{ (x-\theta)y \ge 0\}$ where
$\theta>0$ is a learnt parameter.

The true risk can be explicitely calculated. For $\theta>0$, we have
\begin{align*}
    R_P(\theta) = p \theta^{1 + \alpha} + (1-p) (1-\theta)^{1+\beta},
\end{align*}
and the optimal threshold $\theta^*_{p}$ can be found by derivating the risk
$R_P(\theta)$.  The derivative is zero when $\theta$ satisfies
\begin{align}
    p(1+\alpha) \theta^\alpha = (1-p)(1+\beta)(1-\theta)^\beta.
    \label{optimal_threshold_sim_exp}
\end{align}
Solving \cref{optimal_threshold_sim_exp} is straightforward for well-chosen values of 
$\alpha, \beta$, which are detailed in \cref{fig:tab_sim_exp}. The excess error 
$\mathcal{E}(p',p) = R_P(\theta^*_{p'}) - R_P(\theta^*_{p})$
for the diagonal entries of \cref{fig:tab_sim_exp} are plotted in
\cref{fig:plot_sim_exp}, in the infinite sample case.

% \begin{figure}[h]
%     % \begin{center}
%     \centering
%     \begin{tabular}[h]{lcccc}
% 	\toprule
% 	 $\theta^*_p$ 	& \multicolumn{4}{c}{$\alpha$} \\
% 	 \cmidrule(lr){2-5}
% 	 $\beta$	& 0 & 1/2 & 1 & 2 \\
% 	 \midrule
% 	 \smallskip
% 
% 	 \smallskip
% 	 0 	& $[0,1]$ 
% 	 % & $\min \left( 1, \frac{4}{9}\frac{(1-p)^2}{p^2} \right)$ & 
% 	 & $1\wedge \frac{4}{9}\frac{(1-p)^2}{p^2} \right)$ & 
% 	 $1 \wedge \frac{1-p}{2p} $ & $1 \wedge \frac{(1-p)^2}{9p^2}$\\
% 
% 	 1/2 
% 	 % & $\max\left(0, 1- \frac{4 p^2}{9 (1-p)^2} \right)$ 
% 	 & $0 \vee  \frac{9 - 18p + 5 p^2}{9 (1-p)^2} $ 
% 	 & $\frac{(1-p)^2}{p^2 + (1-p)^2}$ & $1 \wedge
% 	 \left(\frac{9}{32} \frac{(1-p)^2}{p^2} \left[ \sqrt{1 + \frac{64p^2}{9(1-p)^2}} - 1 \right]  \right)
% 	 % 2 \left[ \frac{3}{8} \frac{(1-p)}{p}\right]^2 \left[ \sqrt{1 + \left( \frac{8p}{3(1-p)} \right)^2 } - 1 \right] 
% 	 \right) $ & $\circ$ \\
% 
% 	 \smallskip
% 	 1 	& $0 \vee \frac{2 - 3p}{2(1-p)} $ & $\times$ & $1-p$ & $\times$ \\
% 
% 	 \smallskip
% 	 2 	& $0 \vee \frac{9p - p^2}{9p} $ & $\circ$ & $\times$
% 	 & $\frac{\sqrt{1-p}}{\sqrt{p} + \sqrt{1-p}}$\\
% 	 \bottomrule
%     \end{tabular}
%     % \end{center}
%     \caption{Optimal parameters $\theta^*$ for different values of $\alpha, \beta$.
%     Values at $\times$ are easily found by solving a second order equation, values
%     at $\circ$ require solving a polynomial equation of degree 4.}
%     \label{fig:tab_sim_exp}
% \end{figure}

\begin{figure}[h]
    % \begin{center}
    \centering
    \begin{tabular}[h]{lcccc}
	\toprule
	% $\theta^*_p$
	% \ctoprule(lr){2-5}
	   	& \multicolumn{4}{c}{$(\alpha, \beta)$} \\
	 \cmidrule(lr){2-5}
	 & $(0,0)$ & $(1/2, 1/2)$ & $(1,1)$ & $(2,2)$ \\
	 \midrule
	 \smallskip
	$\theta^*_p$ & $[0,1]$ & $\frac{(1-p)^2}{p^2 + (1-p)^2}$ &
	$1-p$ &  $\frac{\sqrt{1-p}}{\sqrt{p} + \sqrt{1-p}}$\\
	 \bottomrule
    \end{tabular}
    % \end{center}
    \caption{Optimal parameters $\theta^*$ for different values of $\alpha, \beta$.}
    \label{fig:tab_sim_exp}
\end{figure}

\begin{figure}[h]
    \centering

    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/dists/fig_dist_0.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/dists/fig_dist_half.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/dists/fig_dist_1.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/dists/fig_dist_2.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage

    \includegraphics[width=0.5\linewidth]{figures/sim_exp/mats/cbar.pdf}

    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/mats/fig_abs_0.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/mats/fig_abs_half.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/mats/fig_abs_1.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage
    \hfill
    \minipage{0.25\textwidth}
	\includegraphics[width=\linewidth]{figures/sim_exp/mats/fig_abs_2.pdf}
	% \caption*{.}\label{fig:dist_sim_exp}
    \endminipage

    \caption{Pdf's and values of the excess risk $\mathcal{E}(p',p)$ for
    different values of $\alpha, \beta$.}
    \label{fig:plot_sim_exp}
\end{figure}

The results of \cref{fig:plot_sim_exp} show that the optimum for the train 
distribution is significantly different from the optimum for the test distribution
for the excess risk when the problem involves Bayes noise.



\subsection*{Generalities on real data experiments}\label{sec:generalities_expes}

% * Models for the learning process
% * Cost function
% * Parameters for the learning process
% * Explain the graphs, i.e. the test value of the loss
% * Corriger les références à l'appendix dans la rédaction MNIST

\paragraph{Strategy to induce bias in balanced datasets}

In the two real data experiments described in the part concerning the MNIST experiment in the Appendix and in 
\Cref{sec:num}, the same strategy is used to induce class distribution bias or
strata bias. Since both experiments involve a small test dataset, it is kept
intact, while we discard elements of the train dataset to induce bias between
the train and test datasets. The bias is parameterized by a single parameter
$\gamma$, such that when $\gamma$ is close to one, there is little strata or
class bias, while when $\gamma$ approaches $0$, bias is extreme.

The bias we induce is inspired by a power law, which is often used
to model unequal distributions. Each value of a modality, \textit{i.e.} a possible value
of the stratum or class of an instance, is given by one of the values of
the power law at random.
Formally, the target train distribution $\{p_k'\}_{k=1}^K$ over a
modality $S\in\{ 1, \dots, K\}$, is defined for all $1 \le k \le K$ as
\begin{align*}
    p_k' = \frac{\gamma^{- \frac{\lfloor K/2 \rfloor}{\sigma(k)}} p_k}{ 
    \sum_{l=1}^K \gamma^{- \frac{\lfloor K/2 \rfloor}{\sigma(k)}} p_k
},
\end{align*}
where $\sigma$ is a random permutation in $\{1,\dots,K\}$.

To generate a train dataset with modality distribution $\{p_k'\}_{k=1}^K$,
we sample instances from the original train data set $\mathcal{D}_n^\circ=
\{ (X_i', Y_i', S_i') \}_{i=1}^n$, where $Y_i'$ is the class, $S_i'$ is the
modality. For MNIST experiment, $S_i' = Y_i'$, while for \Cref{sec:num},
the value $S_i'$ is the stratum of the instance $i$. The output of the 
train dataset is noted $\mathcal{D}_n$, see \Cref{alg:asymmetric_training_gen}
for the detailed algorithm of the train dataset generation.

\begin{algorithm}[H]
\DontPrintSemicolon
\KwData{$\mathcal{D}_n^\circ = \{ (X_i', Y_i', S_i') \}_{i=1}^n$,
$\{p_k'\}_{k=1}^K$ }
\KwResult{$\mathcal{D}_n$} 

$D \leftarrow \emptyset \qquad  $ 
\emph{\# Initialize the result index set.}


\For{$k=1,\dots,K$}{
    $\mathcal{I}_k \leftarrow \{ i \mid 1 \le i \le n,
    S_i' = k \}\quad $\;
    \emph{\# Count the candidates for each modality.}
}

$m_{\text{samp}} \leftarrow \min (\#\mathcal{I}_1, \dots, \#\mathcal{I}_K) $


\While{$m_{\text{samp}} > 0$}{

    $m_1,\dots,m_K \leftarrow \mathcal{M} (m_{\text{samp}}, p_1, \dots, p_K) $
    $\qquad$ \emph{\# $\mathcal{M}$ is the multinomial law.}
    
    %emph{\# Count the remaining elements for each modality.}

    \For{$k=1,\dots,K$}{
	$D_k \leftarrow \text{RandSet}(m_k, \mathcal{I}_k) $
	$\qquad$ \emph{\# $\text{RandSet}(n, X)$ is a random subset
	of $n$ elements of $X$.}

	$\mathcal{I}_k \leftarrow  \mathcal{I}_k \setminus D_k$
    }
    $m_{\text{samp}} \leftarrow \min 
    \left(\#\mathcal{I}_1, \dots, \#\mathcal{I}_K \right) $

    $ D \leftarrow D \cup \left (\bigcup\limits_{k=1}^{K} D_k \right) $ 
    
 }

 $\mathcal{D}_n \leftarrow \{ (X_i', Y_i', S_i') \mid i \in D \}$

 \textbf{Return} $\mathcal{D}_n$
 \caption{Biased training dataset generation}\label{alg:asymmetric_training_gen}
\end{algorithm}

\paragraph{Models} Both MNIST and ImageNet experiments compare two models: a linear model and a multilayer perceptron (MLP) with
one hidden layer.  Given a classification problem of input $x$ of dimension $d$
with $K$ classes, precisely with $d=784, K=10$ for MNIST and $d=2048, K=1000$
for ImageNet data, a linear model simply learns the weights matrix $W \in
\R^{d\times K}$ and the bias vector $b \in \R^K$ and outputs logits 
$l = W^\top x + b$. On the other hand, the MLP has a hidden layer of dimension
$h = \lfloor(d+K)/2 \rfloor$ and learns the weights matrices 
$W_1\in \R^{d, h}, W_2 \in \{ h, K \}$ and bias vectors $b_1 \in \R^h, 
b_2 \in \R^K$ and outputs logits $l = W_2^\top h(W_1^\top x + b_1) + b_2$
where $h$ is the ReLU function, i.e. $h: x \mapsto \max(x,0)$. The number of 
parameters for each dataset and each model is summarized in
\cref{tab:parameters_model}.
\medskip

\begin{table}[h]
    \centering
    \begin{tabular}{lcc}
	 % \cmidrule(lr){2-3}
	% \ctoprule(lr){2-3}
	\toprule
	& \multicolumn{2}{c}{Model}\\
	 \cmidrule(lr){2-3}
	% \midrule
	Database  & Linear & MLP \\
	\midrule
	MNIST &  7,850 & 315,625 \\
	% (\Cref{sec:MNIST_exp}) 
	\midrule
	ImageNet &  2,049,000 & 4,647,676\\
	% (\Cref{sec:num}) 
	 \bottomrule
	 \\
    \end{tabular}
    \caption{Number of parameters for each model.}
    \label{tab:parameters_model}
\end{table}
The weight decay or l2 penalization for the linear model 
and MLP model are written, respectively
\begin{align*}
    \mathcal{P} = \frac{1}{2} \lVert W \rVert \quad \text{and} \quad 
    \mathcal{P} = \frac{1}{2} \lVert W_1 \rVert + \frac{1}{2} \lVert W_1 \rVert.
\end{align*}

\paragraph{Cost function}
The cost function is the Softmax Cross-Entropy (SCE), which is the most used
classification loss in deep learning. Specifically, given logits $l = 
(l_1,\dots,l_K) \in \R^K$, the softmax function is $\gamma : \R^k \to [0,1]^K$
with $\gamma = (\gamma_1, \dots, \gamma_K)$ and for all $k \in \{1,\dots,K\}$,
\begin{align*}
    \gamma_k : l \mapsto \frac{\exp(l_k)}{\sum_{j=0}^K \exp(l_j)}.
\end{align*}
Given an instance with logits $l$ and ground truth class value $y$, the
expression of the softmax cross-entropy $c(l,y)$ is
\begin{align*}
    c(l,y) = \sum_{k=1}^K \I\{ y = k \} \log \left(\gamma_k(l)\right).
\end{align*}
The loss that is reweighted depending on the cases as described in
\Cref{sec:main} is this quantity $c(l,y)$. The loss on the test set is never
reweighted, since the test set is the target distribution.  The weights and
bias of the model that yield the logits are tuned using backpropagation on this
loss averaged on random batches of $B$ elements of the training data summed
with the regularization term $\lambda \cdot \mathcal{P}$ where $\lambda$ is a
hyperparameter that controls the strength of the regularization. 

\paragraph{Preprocessing, optimization, parameters} 
The images of ILSVRC were encoded using the implementation of ResNet50 provided
by the library \emph{keras}\footnote{https://keras.io/applications/}, 
see \cite{chollet2015keras}, by taking the flattened output of the last
convolutional layer.

Optimization is performed using a momentum batch gradient descent algorithm, which
updates the parameters $\theta_t$ at timestep $t$ with an update vector $v_t$ by
performing the following operations:
\begin{align*}
    v_t &= \gamma v_{t-1} + \eta\nabla C(\theta_{t-1}), \\
    \theta_{t} &= \theta_{t-1} - v_t,
\end{align*}
where $\eta$ is the learning rate and $\gamma$ is the momentum, as explained in
\cite{DBLP:journals/corr/Ruder16}.

The parameters of the learning processes are summarized in \cref{tab:parameters}.
The weight decay parameters $\lambda$ were cross-validated by trying values on a
logarithmic scale, e.g. for ImageNet $\{10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 1\}$ 
and then trying more fine-grained values between the two best results,
e.g. for ImageNet $10^{-3}$ was best and $10^{-2}$ was second best so we tried
$\{ 0.002, 0.003, 0.004, 0.005 \}$. The standard deviation initialization of
the weights was chosen by trial-and-error to avoid overflows. The learning rate
was fixed after trying different values to have fast convergence while keeping
good convergence properties.

\begin{figure}
    \centering
\begin{tabular}[h]{lcc}
    \toprule
    Experiment & MNIST - \Cref{sec:MNIST_exp} & ImageNet - \Cref{sec:num} \\
    \midrule
    Net weights std init $\sigma_0$ & 	0.01 &	0.01 \\
    Weight decay $\lambda$ Unif & 		0.01 & 0.002\\
    Weight decay $\lambda$ Strata & 		X    & 0.003\\
    Weight decay $\lambda$ Class & 		0.01 & 0.003\\
    Weight decay $\lambda$ Sym data & 		X    & 0.001\\
    Learning rate $\eta$ & 		0.01 &	 0.001 \\
    Momentum $\gamma$ &			0.9  &	 0.9 \\
    Batch size $B$ &			1,000 &   1,000 \\
    MLP hidden layer size $h$ &		397 &   1,524 \\
    \bottomrule
\end{tabular}
\caption{Parameters of the MNIST and ImageNet experiments - \Cref{sec:MNIST_exp}
and \Cref{sec:num}.}\label{tab:parameters}
\end{figure}


\paragraph{Stratified information for ImageNet}

In this section, we detail the data preprocessing necessary to assign strata to
the ILSVRC data. These were constructed using a list of 27 high-level
categories found on the ImageNet website\footnote{
\url{http://www.image-net.org/about-stats}} copied in
\Cref{original_categories_imagenet}. 
\begin{figure}
    \centering
\begin{tabular}[h]{lccc}
    \toprule
    categories 		& \# synset & \# images per synset & Total \# images \\
    \midrule
    amphibian		& 94	& 591	& 56K \\
    animal			& 3822	& 732	& 2799K \\
    appliance		& 51	& 1164	& 59K \\
    bird			& 856	& 949	& 812K \\
    covering		& 946	& 819	& 774K \\
    device			& 2385	& 675	& 1610K \\
    fabric			& 262	& 690	& 181K \\
    fish			& 566	& 494	& 280K \\
    flower			& 462	& 735	& 339K \\
    food			& 1495	& 670	& 1001K \\
    fruit			& 309	& 607	& 188K \\
    fungus			& 303	& 453	& 137K \\
    furniture		& 187	& 1043	& 195K \\
    geological formation	& 151	& 838	& 127K \\
    invertebrate		& 728	& 573	& 417K \\
    mammal			& 1138	& 821	& 934K \\
    musical instrument	& 157	& 891	& 140K \\
    plant			& 1666	& 600	& 999K \\
    reptile			& 268	& 707	& 190K \\
    sport			& 166	& 1207	& 200K \\
    structure		& 1239	& 763	& 946K \\
    tool			& 316	& 551	& 174K \\
    tree			& 993	& 568	& 564K \\
    utensil			& 86	& 912	& 78K \\
    vegetable		& 176	& 764	& 135K \\
    vehicle			& 481	& 778	& 374K \\
    person			& 2035	& 468	& 952K \\
    \bottomrule
\end{tabular}
\caption{Original categories used to construct the strata for the experiment of
\Cref{sec:num}.}\label{original_categories_imagenet}
\end{figure}
Each ILSVRC image has a ground truth low level
synset, either from in the name of the training instance, or in the validation 
textfile for the validation dataset, that is provided by the ImageNet website.
The ImageNet API \footnote{\url{http://image-net.org/download-API}}
provides the hierarchy of synsets in the form of \emph{is-a} relationships, e.g.
\emph{a flamingo is a bird}. Using this information, for each synset in the 
validation and training database, we gathered all of its ancestors in the hierarchy
that were in the table \cref{original_categories_imagenet}.
Most of the synsets had only one ancestor, which then accounts for one stratum.
Some of the synsets had no ancestors, or even several ancestors in the table,
which accounts in for extra strata, either a \emph{no-category} stratum or a
strata composed of the union of several ancestors. The final distribution of
the dataset over the created strata is summarized by \Cref{fig:dist_strata_imagenet}.
Observe the presence of a \emph{no\_strata} stratum and of unions of two high-level
synsets strata, e.g. \emph{n00015388\_n01905661}.
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/train_dist_over_strata.pdf}
\caption{Distribution of the ImageNet train dataset over the created strata
which definitions are given in \cref{strata_definitions_imagenet} .}
\label{fig:dist_strata_imagenet}
\end{figure}
A definition provided by the API of each of the synsets involved in the strata
is given in \cref{strata_definitions_imagenet}.
\begin{figure}
    \centering
\begin{tabular}[h]{llll}
    \toprule
    \multicolumn{2}{l}{Strata name} & \multicolumn{2}{l}{Definition}\\
	 \cmidrule(lr){1-2}
	 \cmidrule(lr){3-4}
    % \midrule
n00015388 & n01861778 & animal, animate being, beast (\dots)& mammal, mammalian \\
% brute creature fauna 
no strata & & &\\
\multicolumn{2}{l}{n03183080} & \multicolumn{2}{l}{device} \\
\multicolumn{2}{l}{n03122748} & \multicolumn{2}{l}{covering} \\
\multicolumn{2}{l}{n04524313} & \multicolumn{2}{l}{vehicle} \\
n00015388 &  n01905661 & animal, animate being, beast (\dots)& invertebrate \\
n00015388 & n01503061 & animal, animate being, beast (\dots) & bird \\
n04341686 & & structure, construction & \\
n00015388 & n01661091 & animal, animate being, beast (\dots) & reptile, reptilian \\
n03183080 & n03800933 & device & musical instrument, instrument \\ 
n03405725 &  & furniture, piece of furniture, (\dots) & \\
% article of furniture 
n13134947 & & fruit & \\
n00015388 & n02512053 & animal, animate being, beast (\dots) & fish \\
n07707451 & & vegetable, veggie, veg & \\
n04451818 & & tool & \\
n02729837 & & appliance & \\
n09287968 & & geological formation, formation & \\
n04285146 & & sports equipment & \\
n00015388 & n01627424 & animal, animate being, beast (\dots) & amphibian \\
n07566340 & & foodstuff, food product & \\
n12992868 & & fungus & \\
n04516672 & & utensil & \\
n03309808 & & fabric, cloth, material, textile & \\
n00015388 & & animal, animate being, beast (\dots) & \\
n00017222 & n11669921 & plant, flora, plant life & flower \\
n02729837 & n03183080 & appliance & device\\
n03183080 & n04451818 & device & tool \\
n03122748 & n03183080 & covering & device \\
n04285146 & n04524313 & sports equipment & vehicle \\ 
n04341686 & n04524313 & structure, construction & vehicle \\
n07566340 & n07707451 & foodstuff, food product & vegetable, veggie, veg \\
n03183080 & n04524313 & device & vehicle\\
    \bottomrule
\end{tabular}
\caption{Definitions of the strata created for the experiments in \Cref{sec:num}, 
which frequencies are given in \cref{fig:dist_strata_imagenet}.}\label{strata_definitions_imagenet}
\end{figure}

% TODO: Check this shit, with better optimizers.
% 
% The top-1 accuracy that the original ResNet paper obtain on the validation set
% is $20.75 \%$ and their top-5 accuracy is $5.25$. ---> WEIRD !
 

\subsection*{Classes bias experiment for MNIST}\label{sec:MNIST_exp}

The impact of the bias correction in the multi-class supervised learning
setting described in Section 2 is illustrated on a widely used dataset for
studying classification tasks: the MNIST dataset. 

The MNIST dataset is composed of images $X \in \R^d$ of digits and labels being
the value of the digits. In our experiment, we learn to predict the value of the
digit so we have $K=10$ classes corresponding to digits between $0$ and $9$.
The dataset contains $60,000$ images for training and $10,000$ images for
testing, all equally distributed within the classes. There is therefore
no class bias between train and test samples in the original dataset.

Bias between classes is induced using the power law strategy described
above. We deal with the classification task associated to $(X,Y)$ with a
linear model or a MLP with one hidden layer that optimizes the softmax
cross-entropy (SCE) using momentum gradient descent. We compare the uniform
weighting of each instance in the train set (corresponding to the case where
there is no reweighting described in \cref{eq:emp_risk}) with the reweighting
of each instance using the proportion of each label $Y$ for the train and test
datasets as described in \cref{eq:emp_weighted_risk}. Precisions about the
model and parameters are given in paragraph dealing with \textit{Preprocessing, optimization, parameters} in the Appendix.

The optimization dynamics are summarized in \cref{fig:MNIST_res}. We report
the median over 100 runs of these values for the test set and a fixed random
sample of the train set. For the test set, we represent 95\%
confidence-intervals in a lighter tone. The x-axis corresponds to the number of
iterations of the learning process.

\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/prob_MNIST.pdf}
  % \caption{Probability over classes of test and train.}\label{fig:prob_diff_MNIST}
  \caption*{Comparison of $p_k$'s and $p_k'$'s.}\label{fig:prob_diff_MNIST}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/mnist/linear/quant_cost.pdf}
  % \caption{Learning dynamics without reweighting.}\label{fig:uniform_weights_MNIST}
  \caption*{Linear model: cost.}\label{fig:cost_dyn_MNIST}
  \includegraphics[width=\linewidth]{figures/mnist/mlp/quant_cost.pdf}
  % \caption{Learning dynamics without reweighting.}\label{fig:uniform_weights_MNIST}
  \caption*{MLP model: cost.}\label{fig:cost_dyn_MNIST}
\endminipage\hfill
\minipage{0.32\textwidth}%
    \includegraphics[width=\linewidth]{figures/mnist/linear/quant_acc.pdf}
  % \caption{Learning dynamics for class reweightings.}\label{fig:class_weights_MNIST}
    \caption*{Linear model: miss rate.}\label{fig:miss_dyn_MNIST}
    \includegraphics[width=\linewidth]{figures/mnist/mlp/quant_acc.pdf}
  % \caption{Learning dynamics for class reweightings.}\label{fig:class_weights_MNIST}
    \caption*{MLP model: miss rate.}\label{fig:miss_dyn_MNIST}
\endminipage
\caption{Dynamics for the class reweighting experiment with MNIST.}\label{fig:MNIST_res}
\end{figure}

For the uniform weights, we see that the misclassification rate is pretty low for 
the train set, but poor for the test set. By reweighting the instances, we see that
we favor low error over the test set, which gives a miss probability reduced by
half. 

\subsection{Leveraging different databases}

The Visual Decathlon Challenge considered a resized version of ILSVRC of 72 by 72 pixels.



==> old_expes.tex <==
We now present a few experimental results that
investigate the effectiveness of the approach presented in \cref{sec:method}.
Our first experiment examines the conditions on distributions 
for the sampling weights to be accurate, on a very simple simulated example.
Our second experiment tackles number recognition.
It first uses objective class imbalance to compute sampling weights
for classifying the Street View House Number (SVHN) dataset.
Then, we use a notion of visual similarity to compute weights $\lambda$
for classifying MNIST,
that is measured on the shared deep encoder $g$
or an autoencoder.
Finally, our third experiment addresses racial bias in facial recognition,
and derives weights from a model learned on a database that contains ethnicity information.

\subsection{Empirical Solutions for Sampling Weights}

Before considering image data, we first compute reweighting
functions $\lambda$ on the discrete input space $\Z = \{1, 2\}$,
with simulated data.
In that scenario, we know the distributions and can compare
the true values of the weights $\lambda(k,i)$ 
(those obtained by replacing $\widehat{W}_l$ by $\Omega_l$ in \cref{eq:unormalized-weights}),
with those derived from the minimization of $D_n$.
Our experiments:
1) identifies conditions on the distributions for which
minimizing $D_n$ yields the right importance function,
2) assess the shape of the sampling weights distribution,
since assigning all of the weight on too few observations
risks to jeopardize the generalization ability of our algorithm
in image datasets.
We consider the Gini index of a distribution of weights
to evaluate the repartition of the weights,
as well as have a statistic on the importance function.
The Gini index is an inequality measure that is equal to 0 if weights
are uniformly distributed, and equal to 1 if one sample detains all of the sampling weight.
Formally, it writes $G_{\lambda} = (\sum_{q_1, q_2 \in\Lambda}
\abs{\lambda(q_1) - \lambda(q_2)})/(2n\sum_{q \in \Lambda} \lambda(q))$
for an importance function $\lambda$.

We assume that $K = 2$, and that the test distribution satisfies
$p_{\text{test}}(1) = p_{\text{test}}(2) = 1/2$.
Then, we fix $\omega_1(2) = \omega_2(2) = 1$ and 
$R_k := \omega_k(1) / \omega_k(2) = \omega_k(1)$ for any $k \in \{1, 2\}$.
It implies, for any $k \in \{1, 2\}$,
\begin{align*}
    \Omega_k = \frac{1+R_k}{2} \quad \text{and} \quad
    p_k(1) = \frac{R_k}{1+R_k}.
\end{align*}
Finally, we set $n_1 = 100$ and $n_2 = 100$.

\cref{tab:results-solving-sampling-weights} shows that
the obtained Gini index accurately represents the expected Gini index
as long as either $p_1$ or $p_2$ is not too different from
the testing distribution
($R_1 \in \{0.1, 1, 10\}$ or $R_2 \in \{0.1, 1, 10\}$), 
even if the Gini index is relatively
high (\textit{e.g.} 44 \% for $R_2 = 10^{-2}$ and $R_1 = 10^{-1}$).
However, when both distributions are very similar and different from
the test distribution (\textit{i.e.} $R_1 = R_2 = 10^2$ or $R_1 = R_2 = 10^{-2}$),
the Gini index is not accurate (\textit{i.e.} it has very high variance),
thus we expect poor transfer.
When none of the distributions resembles the target distribution
and the distributions are very different
(\textit{i.e.} $R_1 = 10^2$ and $R_2 = 10^{-2}$ or $R_1 = 10^{-2}$ and $R_2 = 10^2$),
the situation approaches b) in \cref{fig:proba-overlap-assumption}.
In that case, we are unable to recover the optimal weights, even though
they are the uniform weights $\lambda(k,i) = 1/n$ over all observations in our example.

\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{lccccc}
	\toprule
	$R_2$ & $10^{-2}$ & $10^{-1}$ & $1$ & $10$ & $10^2$ \\
	\cmidrule(lr){1-1}\cmidrule(lr){2-6}
	$R_1$ & \multicolumn{5}{c}{Gini index for $\lambda$ computed with $\widehat{W}_k$
	($\times 10^{-2}$)}\\
	\cmidrule(lr){1-1}\cmidrule(lr){2-6}
	$10^{-2}$ & 43 (37) & 45 (12) & 24 (04) 
	& 06 (09) &  26 (08) \\
	$10^{-1}$ &  44 (15) &  40 (09) &  20 (03)
	&  03 (04) &  13 (14) \\
	$1$ & 25 (05) & 20 (03) & 00 (00)& 21 (03)& 25 (04) \\
	$10$ & 05 (06) & 03 (04) & 20 (03) & 39 (09) & 43 (14) \\
	$10^2$ & 26 (09)  & 13 (14) & 25 (05)  & 45 (13) & 44 (42) \\
	\midrule
	$R_1$ & \multicolumn{5}{c}{Absolute difference with true Gini index
	($\times 10^{-2}$)}  \\
	\cmidrule(lr){1-1}\cmidrule(lr){2-6}
	$10^{-2}$ & 17 (24)& 05 (08)& 02 (03)& 03 (06)& 26 (08) \\
	$10^{-1}$ & 06 (10)& 06 (07)& 02 (02)& 03 (04)& 09 (13) \\
	$1$ & 02 (03)& 01 (02)& 00 (00)& 01 (02)& 03 (04) \\
	$10$ & 03 (04)& 03 (04)& 01 (02)& 12 (09)& 06 (11) \\
	$10^2$ & 26 (09)& 09 (13)& 02 (03)& 07 (09)& 19 (27) \\
	\bottomrule
    \end{tabular}
    \caption{
	Gini index of the sampling weights for different values of $R_1$ and $R_2$,
	and absolute difference between the Gini index of weights obtained with
	$\widehat{W}_k$ and that obtained with $\Omega_k$,
	for different values of $R_1$ and $R_2$.
	For both measures, we report the mean and 2 times the standard
    deviation (in parenthesis) over 100 experiments.}\label{tab:results-solving-sampling-weights}
\end{table}

\subsection{Number recognition with different types of bias}\label{subsec:exp-number-reco}

We consider several number recognition databases:
MNIST, MNIST-M, SynNumbers (see \cref{fig:three_types_bias})
and SVHN, as well as the character recognition database not-MNIST
(see \cref{fig:three_types_bias}).
Here, our two experiments have as goals: to solve classification for the SVHN 
database using the others, and then the MNIST database.
SVHN has an uneven distribution on the numbers,
which is used to propose sampling weights for our experiment.
For MNIST, we tried to identify relevant observations
using a similarity measure
% use during training using a deep representation of the numbers.
% measured 
based on the shared deep encoder $g$ output or a shallow autoencoder,
trained to minimize the standard Euclidean distance between the original and
reconstructed image.

All images are resized to the size $32 \times 32$ and MNIST and not-MNIST are converted to RGB
by replicating the $32\times32$ image on the three channels.
Our model consists in a simple network composed of two convolutional layers,
followed by a fully-connected layer that gives a 128-dimensional encoding of the image.
A linear classifier $f_{c(k)}$ finally gives a 10-dimensional output.
We use a different classifier for number recognition and character recognition.
Our loss is the standard softmax cross-entropy.

\textbf{Learning to classify SVHN.}
The SVHN database consists in recognizing house street numbers,
thus naturally contains significant more small numbers (1 to 5)
than high numbers (6 to 9) (see \cref{fig:svhn_summary}).
The class distribution can be precisely estimated by  
considering any good random sample of addresses.
Learning without reweighting the instances gives us a prediction accuracy
of 62\% for SVHN, which is low and should be put in perspective with the 91\%
of \cite{GaninJMLR} obtained with SynNumber and a small sample of SVHN
to transfer deep features.
Our result can be justified by the significant visual difference between the SVHN
images and all of the other databases (\cref{fig:three_types_bias}).
To understand this difference,
we provide the confusion matrix for our model in the left side of \cref{fig:svhn_confusion},
which shows that the prediction 1 accounts for over 1/4th 
(over 0.10/0.38) of overall errors.
We conjecture that the transfer learning procedure of \cite{GaninJMLR}
learns to focus on the central number, while the presence of side numbers
in SVHN combined with the narrowness of the number 1 confuses our network.
We argue that the presence of errors for any couple of
true vs. predicted numbers corroborates that assumption.

Introducing the distribution over the classes $\{ 0, \dots, 10\}$
of dataset $k$ as $\{ q_k^{(0)}, \dots, q_k^{(9)} \}$, \textit{i.e.}
$p_k\left( z \right) = q_k^{(y)}$,
as well as that of $p_{\text{test}}$ as $(q_\text{test}^{(0)}, \dots, q_\text{test}^{(9)})$,
we assume the following biasing functions $\omega_k$ for our source datasets,
\begin{align}\label{eq:sampling-function-svhn}
    \omega_k  : z \mapsto \frac{q_k^{(y)}}{q_\text{test}^{(y)}},
\end{align}
for any $k \in \{1, \dots, 9\}$.
Using the procedure described in \cref{sec:method},
we can derive sampling weights from \cref{eq:sampling-function-svhn}.
The sampling weights naturally give higher weights to
elements of classes 1 and 2, due to their prevalence in the testing
set (\cref{fig:svhn_summary}).
Learning a network with sampling weights gives 
an overall accuracy of 57\%, which is lower than learning without sampling weights.
We provide the associated confusion matrix on the left side of \cref{fig:svhn_confusion},
Since we predict less often high numbers, we make less errors on the top right of 
the left-hand-side confusion matrix in \cref{fig:svhn_confusion}.
However, more than 32\% (over 0.14/0.43) of errors are now wrong number $1$ predictions.
In that experiment, we conclude that reweighting made a specific error more frequent,
event though the proposed reweighting procedure is very natural when dealing
with class imbalance.

% \robin{Follow-up experiment: What happens when I remove the not-MNIST database ?}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.475\columnwidth]{figures/num_exps/svhn_dist.pdf}
    \caption{Small sample and class proportions for SVHN.
    }\label{fig:svhn_summary}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/num_exps/confusion_svhn.pdf}
    \caption{Confusion matrix for our initial model on SVHN (left)
	and that learned with our sampling weights (right).
    }\label{fig:svhn_confusion}
\end{figure}

\textbf{Learning to classify MNIST.}
We learn to classify the MNIST database using the others,
and derive sampling weights for the observations using a notion of visual similarity
between an instance and the expected appearance of MNIST.
To define of visual similarity,
we propose using distances between the low-dimensional encoding
of a training observation and its average over MNIST.
We use two types of low-dimensional encodings.
Our first proposition is a the 128-dimensional encoding $g$ of our model
pre-trained for classification on all databases but MNIST.
Our second proposition is a 32-dimensional encoding from a shallow autoencoder
trained on all databases but MNIST.
We denote by $e_{\text{MNIST}}$ the average encoding on MNIST,
by $e_k$ that of the training database indexed by $k$,
and by $e$ any normalized encoding in $\R^{32}$.
Then, we choose the biasing functions:
\begin{align}\label{eq:expression-omega-mnist}
    % \omega_k:& e \mapsto \exp\left( 
    %     - \beta \cdot e^\top [e_{k} - e_{\text{MNIST}} ]
    % \right),\\
    \omega_k:& e \mapsto \exp\left( 
    - \beta \cdot \left[
	\norm{e - e_{k}}_2^2 - \norm{e - e_{\text{MNIST}}}_2^2
    \right]
    \right),
\end{align}
where $\beta \ge 0$ is a smoothing parameter
and $\norm{\cdot}_2$ is the usual Euclidean norm.
When $\beta = 0$, we recover the uniform sampling weights.
On the other hand, when $\beta$ is large, the weight is
very inequally distributed.
The sampling weights are then obtained by following the procedure of \cref{sec:method}.
Considering different values of $\beta \in [10^{-5}, 10^{-2}]$ for the sampling weights,
our classifiers with non-uniform sampling resulted in classification accuracies
that were the same or lower (when $\beta$ approaches $10^{-2}$) than the original model
(95\% accuracy on the 70K elements of MNIST).
To understand that result, we provide the highest and lowest sampling weights elements
for the two scenarios in \cref{fig:weights_for_mnist}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/num_exps/extreme_weights.pdf}
    \caption{Highest and lowest sampling weights obtained
    using \cref{eq:expression-omega-mnist} with encodings
    derived from a classification model or a simple autoencoder.
    }\label{fig:weights_for_mnist}
\end{figure}

In \cref{fig:weights_for_mnist} and with the classification encoding,
the reweighting procedure assigns high weights to 
images that feature a white background and black objects,
and low weights to images with very saturated colors.
However, the saturated images look very similar visually
to the images of the MNIST dataset, while some of the highest
weighted images do not feature a number at all
(those are from the MNIST-M dataset).
In conclusion, using the classification encoding
and \cref{eq:expression-omega-mnist} seems to favor the images
that share the same color shades with MNIST,
but disregards images that feature recognizable MNIST numbers shapes.

In \cref{fig:weights_for_mnist} and with the autoencoder-based encoding,
the reweighting procedure assigns high weights to 
images that feature a dark number on a light background,
and low weights to images that feature a light character on a
dark background. Again, the reweighting procedure
disregards important information based on ``low-level'' visual differences.
These results motivate us to consider explicitly those differences
in our models, possibly with the approach proposed by \cite{GaninJMLR}.

We argue that defining biasing functions using similarities between feature maps
is a natural approach. Indeed, \cite{DwivediR19} shows that measuring similarity
between feature maps can be used to evaluate transferability across tasks.
However, that approach did not select desired instances in our experiments.

\subsection{Correcting for racial bias in facial recognition}

Unlike in \cref{subsec:exp-number-reco},
correcting for bias in \cref{ex:facial-recognition}
does not aim to improve an objective value.
Indeed, in \cref{ex:facial-recognition},
it aims to correct for differences in recognition accuracy
between sensible groups, identified by some notion of ethnicity.
In this experiment, we use a simple model to classify faces by ethnicity,
and derive sampling weights from that model to learn a corrected face recognition model.
We train our ethnicity classifier using a small sample of ethnicity-labeled images.

The Racial Faces in-the-Wild (RFW) database of \cite{racialfaces}
labeled a subset of the identities of the MS-Celeb-1M (MS1M) dataset \cite{GuoZHHG16}
with some ethnicity information.
Precisely, they chose to classify images between four ethnicities:
African, Asian, Caucasian and Indian.
The distribution of RFW over these four ethnicities
is summarized in \cref{tab:distribution-racialfaces}.
Using a small portion of that labeled data (25\% of identities),
we learn our ethnicity classifier.
The ethnicity classifier is used to derive sampling weights for MS1M
without the RFW images.
We use the version of MS1M 
provided in the Lightweight Face Recognition Challenge \& Workshop of ICCV 2019
\footnote{\href{https://ibug.doc.ic.ac.uk/resources/lightweight-face-recognition-challenge-workshop/}{Link to the data}.}
to learn our facial recognition and ethnicity classification models.
To evaluate our facial recognition model, we generated several
testing scenarios with the remaining 75\% of identities in RFW
(not used to learn the ethnicity prediction model).
Precisely, we generated 5 scenarios:
one where the testing database contains 25\% of each ethnicity (\textit{Balanced})
and four where the testing database contains a majority (90\%) of people
of one ethnicity, while the remaining 10\% is equally distributed on other ethnicities.
We call those scenarios \textit{most-African}, \textit{most-Asian},
\textit{most-Caucasian} and \textit{most-Indian}.

\begin{table}
    \centering
    \begin{tabular}{lcc}
	\toprule
	Ethnicity & \# images & \# identities\\
	\hline
	African & 125,684 & 2,995\\
	Asian & 108,874 & 2,490\\
	Caucasian & 176,313 & 2,958\\
	Indian  & 173,288 & 2,983\\
	\hline \hline
	Total & 584,159 & 11,426\\
	\bottomrule
    \end{tabular}
    \caption{Number of observations of each ethnicity in RFW,
	using the ethnicity-labeled identities in RFW.
	RFW is a subset of the MS-Celeb-1M (MS1M) dataset \cite{GuoZHHG16}.
	MS1M contains 5,179,509 images for 93,431 identities.
    }
    \label{tab:distribution-racialfaces}
\end{table}

The ethnicity predictor minimizes the usual softmax cross-entropy
for classifying ethnicities, and gives 4-dimensional softmax probabilities
$s \in \R^4$.
We provide the confusion matrix for ethnicity prediction
in \cref{fig:confusion_matrix_ethnicity}.
Using this model, we compute the average softmax 
of the training database, denoted as $\bar{s}_{\text{train}}$.
Introducing the proportion of each ethnicity for
a scenario as $\bar{q}_{\text{Scenario}}$,
where \textit{Scenario} is either \textit{Balanced}, \textit{most-African},
\textit{most-Asian}, \textit{most-Caucasian} or \textit{most-Indian},
our biasing function writes
\begin{align}\label{eq:biaising-function}
    \omega_1: s \mapsto \frac{s^\top  \bar{s}_{\text{train}} + \beta}{s^\top q_{\text{Scenario}}
    + \beta},
\end{align}
where $\beta \ge 0$ is a smoothing parameter.
The parameter $\beta$ prevents very unequal weight distributions.
Since setting $\beta = 0$ gave fairly well-distributed weights
in this experiment (see \cref{fig:distribution_learnt_weights}), we simply kept $\beta = 0$.
Additionally, we have $K = 1$, thus \cref{eq:unormalized-weights} simply reduces to:
\begin{align}\label{eq:reweighting-function}
    \lambda(k, i) &= \frac{ \widehat{W}_1}{\omega_1(z_i^{(k)})},
\end{align}
and the $\lambda(k,i)$ are inversely proportional to the $\omega_1(z_i^{(k)})$'s.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/face_exps/confusion_matrix.pdf}
    \caption{(Left) Confusion matrix for our ethnicity prediction model.
	Although the notion of ethnicity used by \cite{racialfaces}
	is arbitrary, our model can split the instances quite accurately.
	Still, some ethnicities are less separable than others.
	(Right) Instance with the highest sampling weight
	for each scenario.}\label{fig:confusion_matrix_ethnicity}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.425\linewidth]{figures/face_exps/distribution_gamma_0.pdf}
    \caption{Distribution of the weights for different objective scenarios,
	using \cref{eq:biaising-function} with $\beta = 0$.
	We see that the weights can be larger for \textit{dom-Indian},
	since the ethnicity Indian is the least represented in the database.
	The weights are more evenly distributed for the Caucasian ethnicity,
	the most represented ethnicity in MSM1.
	The highest weights for the \textit{Balanced} scenario are Indian faces,
	since the associated numerator in \cref{eq:biaising-function} is lower.
    }\label{fig:distribution_learnt_weights}
\end{figure}

Since learning a face recognition model is computationally intensive,
we fine-tuned the weights of a network pre-trained with uniform weights
on the MS1M dataset (without RFW).
The fine-tuning procedure consisted in running gradient descent steps
for a few epochs on the reweighted dataset.
Both of our models (ethnicity predicition and face recognition) used 
a ResNet-14 model for $g$, which outputs $64$-dimensional encodings.
We evaluate the similarity between pairs of observations using
the cosine distance of their encodings.
The $\roc$ curve is the golden standard to evaluate similarity measures,
and represents the true positive rate (TPR) (or the false negative rate (FNR))
as a function of the false positive rate (FPR)
for testing for positive pairs (same identity) by thresholding the similarity.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/face_exps/roc_curves_adapt_large.pdf}
    \caption{ROC curve per ethnicity on the RFW database, before fine-tuning
	and after fine-tuning with reweighting using the \textit{Balanced},
	\textit{most-African},
	\textit{most-Asian}, \textit{most-Caucasian} and \textit{most-Indian} scenarios.
    }\label{fig:roc_curve_after_adapt}
\end{figure}

\cref{fig:roc_curve_after_adapt} provides the $\roc$ curves
for each ethnicity of RFW of a model learnt on all observations of MS1M
but those of RFW.
They are calculated using all positive pairs and a randomly selected sample
of $5\times10^6$ negative pairs.
For the uniform sampling weights and a FPR of $0.1$,
we observe that the ratio between the FNR's for the African
and Caucasian ethnicities is higher than 3.
After fine-tuning for \textit{most-African} it is less than 1.5.
Similarly, all scenarios with a majority ethnicity (all but \textit{Balanced}) 
have a better $\roc$ curve for that ethnicity (lower is better).
In some cases, they have brought the $\roc$ curves of the different ethnicities closer together,
which improves the system with regards to racial bias (see \cref{ex:facial-recognition}).

% since racial statistics raise ethical concerns in many countries.
% However, skin color is an usual proxy to determine the race
% and should explain most of the visual appearance of face recognition
% type images.

% For those reasons, we learn a very low-dimensional autoencoder for face images
% that minimizes the standard Euclidean distance on pixels between the true image
% and the decoded one.
% We can then consider two points in the obtained low-dimensional encoding
% to be close when the original images represent individuals of the same ethnicity,
% and far otherwise.

Our experiments favorized shallow network and simple preprocessing of the data,
making the recognition accuracy displayed in \cref{fig:roc_curve_after_adapt}
not very competitive.
Although our method do not change with the size of the network or different preprocessing steps,
we will consider adjusting these parameters for more competitive results in future work.
While setting $K = 1$ gives the simple reweighting function in \cref{eq:reweighting-function},
we are confident that our methodology can be extended to the case of several training databases,
which is also a direction for future work.
A simple follow-up experiment here is to split the training dataset
to compare the weights obtained with the approach of \cref{sec:method}
with our weights for $K=1$.
Our results (\cref{fig:roc_curve_after_adapt}) show that reweighting
misrepresented ethnicity groups can help to correct for racial bias in facial recognition.
However, changing the representativity of the database is not sufficient in general
(see \textit{Balanced} in \cref{fig:roc_curve_after_adapt}).
In that regard, \cite{vogel2020learning} proposed to introduce explicit fairness constraints
that are directly expressed on $\roc$ curves.

\bigskip

Precisely, we first split the classes $\mathcal{Y} = \{ 1,  \dots, M \}$ into
$K$ groups delimited using the integers $(m_1, m_2) \in \N^* \times [\![ 0, K ]\!]$
that satisfy $M = m_1 \times K + m_2$.


\robin{End merge this}

Introducing an overlap parameter $\gamma \in [0, 1]$, 
we sample elements from the full dataset with replacement with probability, for $\mathcal{D}_1$, 
\begin{align*}
    p_1(y) &:=
    \begin{cases}
	\frac{1}{m_1(1+\gamma)} & \text{ if } y \le m_1, \\
     \frac{\gamma}{m_1(1+\gamma)} & \text{ if } m_1 < y \le 2m_1,\\
     0 & \text{ otherwise.}
    \end{cases}
\end{align*}
for $\mathcal{D}_k$ for all $1 < k < K$,
\begin{align*}
    p_k(y) &:=
    \begin{cases}
	\frac{1-\gamma}{m_1} & \text{ if } (k-1)m_1  < y \le km_1, \\
	\frac{\gamma}{m_1}  & \text{ if } k m_1 < y \le (k+1)m_1,\\
	 0 & \text{ otherwise.}
    \end{cases}
\end{align*}
and for $\mathcal{D}_K$,
\begin{align*}
    p_K(y) &:=
    \begin{cases}
	\frac{1-\gamma}{m_1(1-\gamma + m_2)} 
	 & \text{ if } (K-1)m_1  < y \le Km_1, \\
	 \frac{1}{1-\gamma + m_2} & \text{ if } Km_1 < y,\\
	 0 & \text{ otherwise.}
    \end{cases}
\end{align*}

where $\lfloor \cdot \rfloor$ is the floor function,
$n_K = \lfloor (1-\gamma + m_2) n_2 \rfloor$ and 
$n_k = n_2$ for any $k \in \{ 2, \dots, K-1 \}$.
To force the concatenation of all datasets $\mathcal{D}_1, \dots, \mathcal{D}_K$
to have the same number of points as the original dataset, we also
set $\sum_{k=1}^K n_k = 50,000$.


==> rejected.tex <==
\section{Rejected ideas}

\textbf{Simple expression of the biasing functions.}
While knowing the values of $\omega_k$'s over the input space $\mathcal{Z}$
is unlikely in a practical case,
both \cite{laforgue2019statistical} and \cite{vogel2020weighted}
underlined several practical cases where it has a simple form,
the analysis of the latter being restricted to the case $K = 1$.
Following in the footsteps of \cite{vogel2020weighted},
a natural assumption is to consider the samples $\mathcal{D}_{n_k}^{(k)}$
to contains differents proportions of elements issued
from the target classes $\Y$.
Introducing the proportion of class $l$ in sample $\mathcal{D}_{n_k}^{(k)}$
as $q^{(k)}_l = \p_{Z\sim P^{(k)}} \{ Y = k \}$ and
the distribution associated to class $l$ as $(Z \mid Y = l) \sim Q_l$ for any $(k, l) \in \{1, \dots, K\} \times\Y$, this assumption is expressed formally as
\begin{align}\label{eq:simple-class-basing-fun}
    \forall k \in \{1, \dots, K\} \quad 
    P^{(k)} = \sum_{l=1}^L q^{(k)}_l Q_l.
\end{align}
We introduce the class proportions of the test distribution
as $q_l = \p_{Z\sim P}\{ Y = l \}$.
Under \cref{eq:simple-class-basing-fun}, the biasing functions satisfy:
\begin{align}\label{eq:expression-of-biasing-function}
    \forall k \in \{1, \dots, K\} \; \text{and} \;
    z=(x, y) \in \mathcal{Z},
    \quad 
    \frac{\omega^{(k)}(z)}{\Omega^{(k)}} = \sum_{l=1}^L \I\{ y = l\} \frac{q_l^{(k)}}{q_l}.
\end{align}
The biasing function $\omega^{(k)}(z)$ for $z = (x, y)$ is thus proportional
to the ratio of the expected proportions of class $y$ in $P^{(k)}$ and $P$.
While \cite{laforgue2019statistical} assumes that the biasing function is known,
usually the quantities $q_l^{(k)}/q_l$ for $l,k \in \Y \times \{ 1, \dots, K \}$
are unknown in most situations.
While the quantity $q_l^{(k)}$ can be estimated from the data
there is no sample available to estimate $q_l$.
In that regard, \citep{vogel2020weighted} simply assumes the $q_l$'s
to be known.

\begin{remark}
    \textbf{Reweighting with strata.}
    The notion of objective
    --- such as the classification objective of \cref{eq:Expected_risk} ---
    does not intervene in our reweighting scheme.
    Hence, the biasing functions can be determined on a statification of the data
    that is totally independent of the objective.
    Precisely, \cite{vogel2020weighted} assumed the existence
    of \textit{strata} and the knowledge of strata probabilities
    to derive a reweighting scheme.
    \label{rem:strata}
\end{remark}

\textbf{A natural estimator for $P$.}
Under our \cref{eq:expression-of-biasing-function},
equation (4) of \cite{laforgue2019statistical} gives
\begin{align}\label{eq:dist-theo}
    P(dz) = \left( \sum_{k=1}^K \sum_{l=1}^L \lambda_k  \cdot
    \I\{ y = l \}\frac{q_l^{(k)}}{q_l}  \right)^{-1}
    \cdot \bar{P}(dz),
\end{align}
which implies a natural approximation of $P$ under the assumption
that the $q_l$ are known and that we can estimate the $q_l^{(k)}$ 
from the data. 
Using the sample $\mathcal{D}_{n_k}^{(k)}$, we can estimate
by $\widehat{q}_l^{(k)}$ the quantities $q_l^{(k)}$, with
\begin{align}\label{eq:estimator}
    \widehat{q}_l^{(k)} := (1/n_k) \cdot \sum_{i=1}^{n_k} \I\{ Y_i^{(k)} = l \},
\end{align}
for any $(k,l) \in \{ 1, \dots, K \}\times\{1, \dots, L \}$.
Plugging in \cref{eq:estimator} in \cref{eq:dist-theo} gives the following
empirical estimator $\widehat{P}_n$ for $P$
\robin{TODO: Homogeneiser les notations $\widetilde{P}_n$}
\begin{align*}
    \widehat{P}_n(dz) = \left( \sum_{k=1}^K \sum_{l=1}^L (n_k/n)  \cdot
    \I\{ y = l \}\frac{\widehat{q}_l^{(k)}}{q_l}  \right)^{-1}
    \cdot \widetilde{P}_n(dz),
\end{align*}

\textbf{Determination of the probability ratios.}
Assume the existence of an auxiliary model $h: \X \to \R^{L}$
that outputs some values, such as scores associated to the $L$ classes.
If the model were to assign elements of the input space $\X$ to
a class $\Y$, we could estimate the quantities $q_l^{(k)}$ and $q_l$
for all $(k,l) \in \{ 1, \dots, K \} \times \Y$.
Introduce the following matrices:
\begin{align*}
    H^{(k)} &=
    \begin{pmatrix}
	h\left(X_1^{(k)}\right) \\ \dots \\ h\left(X_{n_k}^{(k)}\right)
    \end{pmatrix} \qquad \text{and} \qquad
    H = \begin{pmatrix}
	h\left(X_1\right) \\ \dots \\ h\left(X_n\right)
    \end{pmatrix},
\end{align*}
with $H^{(k)} \in \R^{n_k \times L}$ for any $k\in\{1, \dots, K\}$
and $H \in \R^{n \times L}$.
A good approximation of the biasing function presented in
\cref{eq:expression-of-biasing-function} evaluated on the point $x \in \X$
is the following expression
\begin{align}\label{eq:expression-of-the-weights}
    \widetilde{\omega}^{(k)}(x) = L \cdot 
     \exp\left( 
	(\gamma_k/n_k) \cdot  \mathbf{1}^\top H^{(k)} 
	 - (\gamma_k/n) \cdot  \mathbf{1}^\top H 
    \right)
    \times \text{soft} \left(\gamma_k \cdot h(x) \right)^\top,
\end{align}
where $\mathbf{1} = (1, \dots, 1)^{\top}$ is the unit vector,
$\text{soft}(v) = \exp(v)/(\exp(v) \times \mathbf{1} )$
is the softmax function and $\gamma_k \in \R_+$ parameterizes
a ressemblance prior between the database $\mathcal{D}_{n_k}^{(k)}$
and the test distribution.
Note that $\gamma_k = 0$ corresponds to a $\widetilde{\omega}^{(k)}(z) = 1$,
thus to the inclusion of an unweighted $\mathcal{D}_{n_k}^{(k)}$ in the training set.
However, as $\gamma_k$ grows, the quantity in \cref{eq:expression-of-the-weights}
is high if $h(x)$ is large on the same coordinates as the sample
$\mathcal{D}_{n_k}^{(k)}$ relatively to the sample $\mathcal{D}_n$,
in an ``average sense''.
The numerical stability of the expression in \cref{eq:expression-of-the-weights}
is assured using the techniques described in \cite[Chapter 4]{Goodfellow2016}.

\section{Practical implementation}

To implement our method in practice, we consider for the auxiliary model
$h$ a selected activation maps of a ResNet-26 convolutional neural network
\citep{He2015}.
This network was pre-trained for classification on the images of
the well-known visual recognition dataset ImageNet \cite{ImageNetDB},
in a resized version made for the Visual Domain Decathlon set of datasets
\citep{VisualDomainDecathlon}.
Our experiments will evaluate the ability and success of our method
for learning models specialized for some databases of the Visual Domain
Decathlon datasets using data from other databases of it.

\robin{
    \begin{itemize}
	\item Which level of activation maps to chose ?
	\item How to retrain the network, if I don't retrain it from scratch ?
	\item Add visualizations of the weights of each databases,
	    for different values of $\gamma_k$.
	\item How to choose the databases to use in my training process ?
	    Use the scalar product of the caracteristic probability vectors
	    associated. Not very clear, but see the formula above.
    \end{itemize}
}

\textbf{Databases.}
\robin{
    Ajouter une description rapide des bases principales
    du Visual Domain Decathlon challenge.
}


\section{Practical Methods}

\section{Experimental Results}

\robin{Réponse expérimentales aux questions ci-dessus.}

\robin{Limites et extensions à d'autres domaines comme la reconnaissance faciale,
avec des prédicteurs de race/genre.}

